Emora STDM: A Versatile Framework for Innovative Dialogue System Development

This demo paper presents Emora STDM (State Transition Dialogue Manager), a dialogue system development framework that provides novel workflows for rapid prototyping of chat-based dialogue managers as well as collaborative development of complex interactions. Our framework caters to a wide range of expertise levels by supporting interoperability between two popular approaches, state machine and information state, to dialogue management. Our Natural Language Expression package allows seamless integration of pattern matching, custom NLP modules, and database querying, that makes the workflows much more efficient. As a user study, we adopt this framework to an interdisciplinary undergraduate course where students with both technical and non-technical backgrounds are able to develop creative dialogue managers in a short period of time.

==> tables_and_figures/composite.tex <==

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{blue},
  stringstyle=\color{blue},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

\begin{lstlisting}[caption={Composite Dialogue System}]

# create two independent dialogue modules
df1 = DialogueFlow('start_1')
df1.add_transitions('df1.json')
df2 = DialogueFlow('start_2')
df2.add_transitions('df2.json')

# compose the modules into a single system
cdf = CompositeDialogueFlow('start')
cdf.add_module(df1, 'DF1')
cdf.add_module(df2, 'DF2')
cdf.add_user_transition(
    ('DF1', 'stateA'), ('DF2', 'stateB'), 
    "[{film, movie}]")
cdf.run()

\end{lstlisting}

==> tables_and_figures/information_state_json.tex <==

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{blue},
  stringstyle=\color{blue},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

\begin{lstlisting}[caption={JSON Format for Update Rules}]
{
  "[$user_favorite=#MDB() my favorite]":
      "#ASSIGN($user_like=$user_favorite)",
  "#IF($user_like != None)": 
      "I like $user_like too! (0.5)"
}
\end{lstlisting}

==> tables_and_figures/natex.tex <==

\begin{table}[htbp!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{l||c|c}
	\bf User Input $\rightarrow$ \NATEX & \bf Match & \bf \textsc{\$movie} \\ \hline\hline
	Did you ever watch Avengers?        &  \cmark   &       Avengers       \\ \hline
	Have you seen Star Wars recently?   &  \cmark   &      Star Wars       \\ \hline
	I want to watch Avengers            &           &                      \\ \hline
%	You have to watch Star Wars         &           &                      \\ \hline
	Have you seen the latest news?      &           &
\end{tabular}}
\caption{Classification results for the following \NATEX\LN [\{\textit{have}, \textit{did}\} \textit{you} \{\textit{seen}, \textit{watch}\} \textsc{\$movie}=\texttt{\#MDB()}] against various user inputs in natural language.}
\label{tab:natex}
\end{table}

==> tables_and_figures/natex_regex_compilation.tex <==

\begin{table}[htbp!]
\centering\small{
\begin{tabular}{c||c}
Input & Match \\
\hline
\hline
 A B & A B \\
\hline
 [A, B] & .*?\textbackslash bA\testbackslash b.*?\tesbackslash bB\textbackslash b.*? \\
\hline
 \{A, B\} & \textbackslash\testbackslash b(?:A$|$B)\textbackslash\testbackslash b \\
\hline
 $<$A, B$>$ & .*?(?=.*?\textbackslash bA\textbackslash b).*?(?=.*?\textbackslash bA\textbackslash b).*? \\
\hline
 \$A=B & (?P$<$A$>$B) \\
\hline
 \#F(A, B) & \textit{return value of function F} \\
\end{tabular}}
\caption{Syntax for Natex and corresponding Regex form after compilation}
\label{tab:avgs}
\end{table}

==> tables_and_figures/python_example.tex <==

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

\begin{lstlisting}[float=*]

df = DialogueFlow('root', initial_speaker=DialogueFlow.Speaker.USER)

df.add_user_transition('root', 'initiation_state',
    "[I, {saw, watched} $movie=#MOVIELOOKUP()]")
df.add_system_transition('initiation_state', 'response_state',
    "I've seen $movie too. {Did you like it?, You liked it, right?}")
df.add_user_transition('initiation_state', 'like_state',
    "{#SENT(positive), [yes]}")
df.add_user_transition('initiation_state', 'dislike_state',
    "{#SENT(negative), [no]}")
df.set_error_successor('initiation_state', 'error_state')
df.add_system_transition('error_state', 'response_state',
    "Sorry, I didn't catch that. Did you like $movie?")

\end{lstlisting}



==> tables_and_figures/state_machine_json.tex <==

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{blue},
  stringstyle=\color{blue},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

\begin{lstlisting}[caption=JSON Format for Dialogue Graph]

{
  "Have you seen any good movies lately?": {
    "state": "c",
    "[-movies, I, $e=#ONT(entertainment]": {
      "Oh, so what's your favorite $e?": {}
    },
    "[$movie=#MDB()]":{
        "$movie is one of my favorites!": {}
    }
    "error": {
        "Sorry, I didn't catch that.": "c"
    }
  }
}

\end{lstlisting}


==> tex/demo_description.tex <==

\section*{Emora STDM Demonstration}

The primary objective of our demonstration is to convey the scope of capabilities of our new open-source dialogue development framework, Emora STDM. To meet this objective, our demo is structured as a presentation-style dialogue system development walkthrough. We show step-by-step examples of how a robust dialogue system capable of complex interactions with users can be rapidly developed within our framework. Each step of our sample development process highlights a key feature of our framework. We emphasize how notorious challenges in dialogue development, such as classifying user input, transitioning between topics, etc. can be tackled directly by our framework with minimal developer effort. 

A brief outline of our demonstration of dialogue system development within Emora STDM is as follows. First, we will show the speed with which a simple dialogue system can be constructed, using pattern matching for natural language understanding (NLU) and a state machine for dialogue management. We then show how pattern matching NLU can be seamlessly integrated with NLP models to improve input classification and information extraction. We then show how developers can integrate arbitrary custom logic, including database look-ups, into their system. To improve the flexibility of conversation, we demonstrate how information state theory can be incorporated into dialogue management. Finally, we give an example of how independent dialogue systems can be combined into a larger dialogue agent with greater topic coverage.

\subsection{Equipment Needed}

Since our demonstration is formatted as a presentation, equipment needs are similar to that of a standard presentation setting. We do request a standing-height surface for the presenter's 17-inch laptop. The presenter will use their own laptop to project visual aids to a presentation screen, which requires an HDMI connection for screen mirroring.

\subsection{Intended Impact}

We believe our demonstration is especially useful to two target SigDial audience groups. First, researchers who are interested in dialogue research, but do not have extensive time or interest in developing complete dialogue systems from the ground up, may benefit from our demonstration to learn efficient methods for dialogue system development. Our demonstration illustrates many known practical challenges and corresponding best practices for dialogue system development, and aims to prove that developing a sophisticated dialogue system can be a speedy process given the proper tools and development approach. Second, researchers who are directly interested in dialogue management and practical challenges to dialogue development are likely to find compelling new ideas in our framework's design, which are outlined out paper. Lastly, we hope that broadcasting our framework and its features will directly translate into savings of man-hours and debugging efforts for anyone who adopts Emora STDM for their own development.






==> tex/workflow.tex <==

\section{Workflow}




%Add transitions.

%JSON format in FIGURE.

%Library makes integration easy.

%Serialize/deserialize for deployment.

%The main task in developing a dialogue system using the Emora STDM framework is to add user and system transitions into the dialogue graph. This can be done either using corresponding function calls in the Python API or by constructing and loading a JSON file specifying the transitions of a dialogue graph. Similarly, the Knowledge Base (including the Ontology) can be updated using either API calls or by loading a JSON file. Implementation of our framework as Python library makes it convenient to integrate within a larger application or within an automated evaluation setting. In cases where a user wishes to deploy a dialogue system in a web application or web API, our framework provides straightforward serialization and deserialization functions to track dialogue state between requests. 




%\input{tables_and_figures/json_example}
%\input{tables_and_figures/python_example}


%\subsection{Error Handling}

%Error transitions.

%Accumulate and report unexpected input.

%Automatic recovery attempts from errors. (skipped)

%One of the primary challenges of constructing any dialogue system is how to handle unexpected user input. Our framework addresses this challenge directly by providing a mechanism known as error transitions, which are taken when a user input does not match the Natex of any outbound transition. This allows a dialogue system to have a systematic and graceful recovery from input that the designer did not anticipate. 

%Dialogue system development often involves more time and effort spent on improving an existing system, rather than the initial system design. Identifying the cases in which the dialogue system lacks coverage in user input interpretation can be costly. To aid the process of improving what inputs a dialogue system can handle, any user input that results in an error transition being taken will automatically log the interaction in a concise report. This reporting mechanism allows a developer to quickly identify unhandled cases and make the appropriate adjustments to the system design.


%\subsection{Transition Control}

%Automatic novelty preference.

%Global transitions.

%Multi-hop transitions. (skipped)

%A major limitation to state-machine-based dialogue managers is their inflexibility, especially when transitioning abruptly to a new topic of conversation at the user request. We mitigate this issue by explicitly supporting \textit{global user transitions}, which can be specified once by the developer to add user transitions with a given Natex between all states of the dialogue graph to a specific target state. This allows a transition to that target state to be evaluated regardless of the current state of the dialogue. 

%Another concern of rule-based dialogue management systems is repetitiveness (i.e. when returning to a particular dialogue state results in repeating a system response from earlier in the dialogue history). Our framework addresses this issue in two ways. First, generation of the system response from Natexes automatically creates variation in the system response (Section X). Second, our system automatically tracks the history of transitions taken in each state in the dialogue graph. Upon returning to that state, the dialogue manager will always prefer to take a transition that is has not recently taken from that state, as long as novel transition options exist. 

%\subsection{Information State Control}

%Supports both state machine and information state approaches to dialogue management.

%Tight interoperability between approaches improves flexibility.

%Information state updates can be made every turn using THING.




%\subsection{Combining Dialogue Components}

%Team development improved by dialogue components.

%Components are encapsulated by namespacing and robust to errors.

%Dialogue system development is often performed in a team-based setting, where individual members are each responsible for developing a separate component of the overall system. Our dialogue development framework has explicit support for combining multiple independent dialogue systems. Independent dialogue graphs and knowledge bases are combined by automatically prepending a namespace tag to each dialogue graph state identifier and knowledge graph node identifier. Dialogue graph transitions can then be added between arbitrary states of two dialogue graph components simply by referencing the state identifiers with the namespace corresponding to the components. This avoids any naming conflicts between dialogue components and the knowledge graphs they rely on, while allowing seamless cross-referencing in the overall architecture. 




